UniHOPE: A Unified Approach for Hand-Only and Hand-Object Pose Estimation

Estimating the 3D pose of hand and potential hand-held object from monocular images is a longstanding challenge. Yet, existing methods are specialized, focusing on either bare-hand or hand interacting with object. No method can flexibly handle both scenarios and their performance degrades when applied to the other scenario. In this paper, we propose UniHOPE, a unified approach for general 3D hand-object pose estimation, flexibly adapting both scenarios. Technically, we design a grasp-aware feature fusion module to integrate hand-object features with an object switcher to dynamically control the hand-object pose estimation according to grasping status. Further, to uplift the robustness of hand pose estimation regardless of object presence, we generate realistic de-occluded image pairs to train the model to learn object-induced hand occlusions, and formulate multi-level feature enhancement techniques for learning occlusion-invariant features. Extensive experiments on three commonly-used benchmarks demonstrate UniHOPE's SOTA performance in addressing hand-only and hand-object scenarios. Code will be released on https://github.com/JoyboyWang/UniHOPE_Pytorch.

==> figures/tex/control_strengths.tex <==
\begin{figure}[t]
    % \centering
    \includegraphics[width=\linewidth]{figures/img/control_strengths.pdf}
    \caption{Our high-quality sample selection strategy. Note the fingers in the yellow box are not aligned with the depth map.}
    \label{fig:control_strengths}
\end{figure}

==> figures/tex/generated_images.tex <==
\begin{figure}[t]
    % \centering
    \includegraphics[width=\linewidth]{figures/img/generated_images.pdf}
    \caption{The generated hand images under various occlusion conditions.}
    \label{fig:generate_images}
\end{figure}
